Discrete Diffusion Schr\"odinger Bridge Matching for Graph Transformation

Transporting between arbitrary distributions is a fundamental goal in generative modeling. Recently proposed diffusion bridge models provide a potential solution, but they rely on a joint distribution that is difficult to obtain in practice. Furthermore, formulations based on continuous domains limit their applicability to discrete domains such as graphs. To overcome these limitations, we propose Discrete Diffusion Schr\"odinger Bridge Matching (DDSBM), a novel framework that utilizes continuous-time Markov chains to solve the SB problem in a high-dimensional discrete state space. Our approach extends Iterative Markovian Fitting to discrete domains, and we have proved its convergence to the SB. Furthermore, we adapt our framework for the graph transformation, and show that our design choice of underlying dynamics characterized by independent modifications of nodes and edges can be interpreted as the entropy-regularized version of optimal transport with a cost function described by the graph edit distance. To demonstrate the effectiveness of our framework, we have applied DDSBM to molecular optimization in the field of chemistry. Experimental results demonstrate that DDSBM effectively optimizes molecules' property-of-interest with minimal graph transformation, successfully retaining other features. Source code is available $\href{https://github.com/junhkim1226/DDSBM}{here}$.

==> 03_theoretical_background.tex <==
\section{Theoretical Background}

\textbf{Notations.}
We consider the \textit{sample space} $\Omega = D([0,\tau], \mathcal{X})$, which is set of all left limited and right continuous (c\`adl\`ag) paths over the finite metric space $(\mathcal{X}, d_{\mathcal{X}})$.
The space of \textit{path measures} is denoted by $\mathcal{P}(\Omega)=\mathcal{P}(D([0, \tau], \mathcal{X}))$.
The subset of \textit{Markov} measures of which the transition probability are continuous and differentiable for time is denoted by $\mathcal{M}$.
The \textit{transition probability} from state $x$ at time $s$ to state $y$ at time $t$ will be represented by $P_{s:t}(x,y)$. 
Similarly, the \textit{transition rate} or \textit{generator} of a Markov measure as $A_{s}(x, y)$.
For any $M\in\mathcal{M}$, the \textit{reciprocal class} of $M$ is denoted by $\mathcal{R}(M)$
(see \cref{def:reciprocal projection}).
For any $\mathbb{P}\in\mathcal{P}(\Omega)$, $\mathbb{P}_{t}$ denotes the marginal distribution at time $t$, $\mathbb{P}_{s, t}$ as the joint distribution at time $s$ and $t$, $\mathbb{P}_{t\vert s}$ the conditional distribution at time $t$ given state at time $s$.
$X = (X_{t})_{t\in[0, \tau]}$ denotes the canonical process given by $X_t(\omega) = \omega_t$ for $\omega = (\omega_s)_{s \in [0,\tau]}\in\Omega$.
The reference measure $\mathbb{Q}\in\mathcal{M}$ is an irreducible Markov measure on $\Omega$ with its associated canonical filtration. 
We will denote the transition rate (or probability) of any Markov measures $M$ other than $\mathbb{Q}$, using a superscript notation.

\subsection{Schr\"odinger Bridge Problem}

% 유클리드 공간에서의 standard Brownian 모션 $(X_t)_{0\le t \le \tau}$ 이 reference로 주어져 있어서, transition density 가 정해져 있다고 생각 해 보자.
% $X_0$ 의 분포, 즉 Initial distribution 이 $\Gamma$로 주어진다면, $X_\tau$ 에서의 분포는 $\Gamma$ 와 transition density 에 의해 결정이 된다.
% Suppose we prescribe in advance not only a initial distribution $\Gamma$, but the terminal distribution of $X_\tau$ as well. 
% Schr\"odinger bridge problem 은 이러한 boundary terminal condition을 만족하면서, 가장 reference process 와 유사한 new process 를 construct 하는 것이다.

Schr\"odinger Bridge (SB) problem is finding a stochastic process that most closely resembles a given reference process, with a condition that initial and final marginal distributions are fixed as $\Gamma$ and $\Xi$.
Specifically, the reference process with the law $\mathbb{Q}$ is given, the optimality is achieved by minimizing Kullback-Leibler (KL) divergence to the reference process, $D_{\text{KL}}(\mathbb{P}\Vert\mathbb{Q})$.
Thus the definition of the SB solution is as below:
\begin{equation}\label{eq:1 DSB definition}
    \mathbb{P}^{\text{SB}}= \arg\min_{\mathbb{P}} \{ D_{\text{KL}}(\mathbb{P}\Vert\mathbb{Q}): \mathbb{P}_{0}=\Gamma, \mathbb{P}_{\tau}=\Xi\}.
\end{equation}

If we additionally fix the initial and terminal coupling $\mathbb{P}_{0,\tau}$, the optimality can be found easily as a mixture of bridges $\mathbb{P}_{0,\tau}\mathbb{Q}_{\cdot\vert 0,\tau}$, which implies that finding the SB solution is equivalent to finding optimal coupling $\mathbb{P}_{0,\tau}^{\text{SB}}$ \citep{leonard2013survey}.
In particular, such optimal coupling is called static SB solution, which could be defined as follows:
\begin{equation}\label{eq:2 SSB definition}
    \mathbb{P}_{0,\tau}^{\text{SB}}=\arg\min_{\mathbb{P}_{0,\tau}}\{D_{\text{KL}}(\mathbb{P}_{0,\tau}\Vert \mathbb{Q}_{0,\tau}): \mathbb{P}_{0}=\Gamma, \mathbb{P}_{\tau}=\Xi\}.
\end{equation}

Note that the KL-divergence is decomposed into the entropy term $H(\mathbb{P}_{0,\tau})$ and the cross-entropy term $\mathbb{E}_{\mathbb{P}_{0,\tau}}\left[-\log q(x_\tau \vert x_0)\right]$, where $q$ denotes the density function of $\mathbb{Q}$.
The cross-entropy term is represented as $L^2$ distance when the $\mathbb{Q}$ is associated with the reversible Brownian motion.
In general, the static SB problem is equivalent to the entropy-regularized optimal transport (EOT) problem with the cost function $c(x, y)=-\log q_{\tau\vert 0}(y \vert x)$ \citep{leonard2013survey}.
While previous approaches have primarily focused on solving SB problems in continuous spaces, typically involving Brownian motion, our work differs by addressing SB solutions in discrete spaces, specifically dealing with c\'adl\'ag paths.
Despite this distinction, the core idea remains rooted in the intrinsic properties of the SB solution (see \cref{theorem:SB solution}).



\subsection{Solution Method}

To solve the SB problem, we adopted the Iterative Markovian Fitting (IMF) method, a technique that has been proposed in various studies \citep{peluchetti2023diffusion, shi2024diffusion}.
These works primarily address diffusion processes in Euclidean space, whereas our approach differs slightly as we focus on a continuous-time Markov chain over finite state space. 
Applying IMF to c\`adl\`ag paths in discrete spaces requires additional theoretical developments or modifications to ensure proper convergence and stability in this new context, which is described in \cref{appendix.a}.

The SB solution is a mixture of pinned-down measures of $\mathbb{Q}(\cdot\vert X_0=x_0, X_\tau=x_\tau)$, where the pair $(x_0, x_\tau)$ is drawn from the coupling $\mathbb{P}_{0,\tau}^{\text{SB}}$.
Based on this, the projection method first constructs a reciprocal measure, which is mixture of pinned-down processes from a given initial coupling.
Although each pinned-down process is Markov, the mixture generally loses the Markov property in general as collection of Markov process is non-convex \citep{leonard2014reciprocal}.
Thus, it then identifies the Markov measure that is closest to the mixture.
This yields an improved coupling, and the process is iterated to obtain a measure that is both the mixture of pinned-down measures and Markov-- the desired SB solution.

In this context, we define the reciprocal projection to describe the construction of a reciprocal mixture from a given coupling (see \cref{def:reciprocal projection}). 
Similarly, the term Markov projection is used to describe the approximation of a reciprocal process with a Markov process (see \cref{def:Markov projection}).
\begin{definition}\label{def:reciprocal projection}
    (Reciprocal Projection)\\
    $\Lambda \in \mathcal{P}(\Omega)$ is in the reciprocal class $\mathcal{R}(\mathbb{Q})$ with respect to a Markov measure $\mathbb{Q}$ if $\Lambda=\Lambda_{0,\tau}\mathbb{Q}_{\vert 0,\tau}$.
    For a measure $\Lambda \in \mathcal{P}(\Omega)$, its reciprocal projection with respect to $\mathbb{Q}$ is 
    $$\Pi_{\mathcal{R}(\mathbb{Q})}(\Lambda)(\cdot):=\iint_{(\cdot)} \Lambda(dx_{0}, dx_{\tau}) \mathbb{Q}(dx_{t}\vert x_{0},x_{\tau}).$$
\end{definition}
Among the measures with the coupling $\Lambda_{0,\tau} \ne \mathbb{P}^{\text{SB}}_{0,\tau}$, the minimizer of the KL-divergence to the reference process is the (non-Markov) reciprocal projection $\Pi_{\mathcal{R}}(\Lambda)$. 
The reciprocal projection consists of a mixture of bridges, where each bridge is derived from Doob’s h-transform with the realization of an end-point pair $(x, y) \sim \Lambda_{0,\tau}$ \citep{levin2017markov}. 
Obviously, it preserves the initial-terminal coupling. 
Although each pinned-down bridge is Markov (see \cref{lemma:h-transform}), the mixture is generally not Markov.
\begin{definition}\label{def:Markov projection}
    (Markov Projection) \\
    Given a path measure $\Lambda\in \mathcal{R}(\mathbb{Q})$, a Markov path measure that minimizes the reverse KL-divergence to $\Lambda$ is called as Markov projection of $\Lambda$,  
    $$\Pi_{\mathcal{M}}(\Lambda)=\arg\min_{M}\left\{D_{\text{KL}}(\Lambda\Vert M): M\in \mathcal{M}\right\}.$$
\end{definition}
The Markov projection preserves the marginal distribution at all times $t$, but does not preserve the coupling.
Furthermore, the generator and the reverse KL-divergence of the Markov projection over c\'adl\'ag paths are explicitly derived in the \cref{prop:Markov projection}.


For a given reciprocal process $\Lambda^{(0)}\in\mathcal{R}(\mathbb{Q})$, we consider a sequence $(\Lambda^{(n)})_{n\in\mathbb{N}}$ which is defined by the recurrence relation:
\begin{align} \label{eq:iterative projection of measures}
    \Lambda^{(2n+1)}&=\Pi_{\mathcal{M}}(\Lambda^{(2n)}),\\ \nonumber
    \Lambda^{(2n+2)}&=\Pi_{\mathcal{R}(\mathbb{Q})}(\Lambda^{(2n+1)}), \nonumber
\end{align}
where $\Lambda_{0}^{(0)}=\Gamma$ and $\Lambda_{\tau}^{(0)}=\Xi$.
Under mild assumptions, the resulting sequence of measures of iterative projection converges to $\mathbb{P}^{\text{SB}}$ in law (see \cref{theorem:convergence,appendix.a.proof of convergence}).

\begin{theorem}\label{theorem:convergence}
    (Convergence of Iteration)\\
    Assume that $D_{\text{KL}}(\Lambda^{(0)}_{0,\tau}\Vert \mathbb{P}^{\text{SB}}_{0, \tau})< \infty$, $\Lambda^{(n)}\ll \mathbb{P}^{\text{SB}}$ for all $n\in \mathbb{N}$. 
    Then the sequence of KL-divergence to $\mathbb{P}^{\text{SB}}$ non-increasing,
    \begin{equation}
        D_{\text{KL}}(\Lambda^{(2n)}\Vert \mathbb{P}^{\text{SB}}) \geq D_{\text{KL}}(\Lambda^{(2n +1)}\Vert \mathbb{P}^{\text{SB}}) \geq D_{\text{KL}}(\Lambda^{(2n + 2)}\Vert \mathbb{P}^{\text{SB}}). \nonumber
    \end{equation}
    $D_{\text{KL}}(\Lambda^{(2n)}\Vert \mathbb{P}^{\text{SB}}) = D_{\text{KL}}(\Lambda^{(2n +1)}\Vert \mathbb{P}^{\text{SB}})$ if and only if $\Lambda^{(2n)}=\Lambda^{(2n+1)}=\mathbb{P}^{\text{SB}}$.
    Moreover, $\Lambda^{(n)}$ converges to $\mathbb{P}^{\text{SB}}$ in law as $n \to \infty$.
\end{theorem}

==> 04_methods.tex <==
\section{Methods}

Here, we propose the Discrete Diffusion Schr\"odinger Bridge Matching (DDSBM) framework, which focuses on solving the SB problem in discrete state spaces.
Approaches to the SB problem in continuous spaces model probability flows through stochastic differential equations, while our method uses continuous-time Markov chains (CTMCs) in discrete state spaces, governed by the Kolmogorov equation \cref{eq:Kolmogorov forward equation}.
We first provide the algorithm of DDSBM (\cref{subsection:Algorithm for Solving the Schrodinger Bridge Problem}) to apply Iterative Markovian Fitting (IMF) to c\`adl\`ag paths in discrete spaces, of which the convergence is ensured theoretically by \cref{theorem:convergence}.
We then discuss how DDSBM can be implemented in the graph transformation (\cref{subsection:process on molecular graph}) and introduce a graph permutation matching algorithm for efficiency (\cref{subsection:graph permutation matching}).


\subsection{Algorithm for Solving the Schr\"odinger Bridge Problem}
\label{subsection:Algorithm for Solving the Schrodinger Bridge Problem}
In this section, we present the framework for solving the SB problem in discrete state spaces based on the IMF algorithm proposed by \citet{shi2024diffusion}.
We refer to it as the DDSBM framework.
The framework iteratively applies Markov and reciprocal projections to update the sequence of measures, as described in \cref{eq:iterative projection of measures}.


It begins with an initial random coupling $\pi$ such that $\pi_0 = \Gamma$ and $\pi_\tau = \Xi$.
Following the definition of the reciprocal class in \cref{def:reciprocal projection}, we construct the initial reciprocal bridge to obtain the measure $\Lambda^{(0)}$.

Given a reciprocal measure $\Lambda^{(2n)} \in \mathcal{R}(\mathbb{Q})$, the next step is to compute its Markov projection $M^{(2n+1)} := \Pi_{\mathcal{M}}(\Lambda^{(2n)})$.
The exact form of the transition rate for $M^{(2n+1)}$ is provided in \cref{prop:Markov projection}.
In practice, the transition rate is approximated by a neural network.

To achieve this, it first samples pairs $(x_0, x_\tau)$ from $\Lambda_{0,\tau}^{(2n)}$ and samples intermediate states $x_t$ by constructing the bridge $\mathbb{Q}(\cdot \vert X_0, X_\tau)$.
The sampled pairs $(x_t, x_\tau)$ are distributed according to $\Lambda_{t,\tau}^{(2n)}$.
Using these realizations, the rate matrix of $M^{(2n+1)}$ is approximated by parameterized Markov measure $M^\theta$, by minimizing the following loss function:
\begin{equation} \label{eq:Loss of forward Markov prjection}
    \mathcal{L}(\theta) =\int_0^\tau \mathbb{E}_{\Lambda_{t,\tau}^{(2n)}} \left[ (A_t^{\mathbb{Q}_{\cdot \vert \tau}} - A_t^{M^\theta})(X_t, X_t) + \sum_{y\ne X_t} A_t^{\mathbb{Q}_{\cdot \vert \tau}}\log{\frac{A_t^{\mathbb{Q}_{\cdot \vert \tau}}}{A_t^{M^\theta}}}(X_t, y)\right]dt,
\end{equation}
where $A_t^{\mathbb{Q}_{\cdot \vert \tau}}$ denotes the generator of pinned down process of $\mathbb{Q}(\cdot\vert X_\tau)$.
From the approximated generator $A_t^{M^\theta}$, we can sample $x_\tau$ given $x_0$, where $(x_0, x_\tau) \sim M^{\theta}_{0,\tau}\approx M^{(2n+1)}_{0,\tau}$.
Note that, until the sequence of measures converges, the new joint coupling $M^\theta_{0,\tau}\approx M^{(2n+1)}_{0,\tau}$ will differ from the previous one $\Lambda_{0,\tau}^{(2n)}$.

Once the Markov measure $M^{(2n+1)}$ is obtained, we proceed to compute the corresponding reciprocal measure $\Lambda^{(2n+1)}$ through reciprocal projection, $\Lambda^{(2n+1)} := \Pi_{\mathcal{R}(\mathbb{Q})}(M^{(2n+1)})$.
In theory, as shown in \cref{prop:Markov projection}, the time marginal distributions are preserved under Markov projection, meaning that $\Lambda^{(2n)}_t = M^{(2n+1)}_t$ for all $t\in[0,\tau]$. 
However, in practice, since the Markov projection is approximated using a neural network, repeatedly applying this approximation can lead to an accumulation of errors in the time marginals.
Such accumulated errors may violate the marginal condition of the SB problem, particularly leading to a potential failure in satisfying the terminal condition $\mathbb{P}_\tau = \Xi$.

To compensate these errors, the next Markov measure $M^{(2n+2)}:=\Pi_{\mathcal{M}}(\Lambda^{(2n+1)})$ is approximated in a time-reversal way (see \cref{prop:Time-reversal Markov projection}).
Based on the time-symmetric nature of Markov measures, we can leverage the time-reversed generator $\tilde{A}_t^{M^{(2n+2)}}$, which enables the sampling of $x_0$ conditioned on $x_\tau$, where $(x_0, x_\tau)\sim M^{(2n+2)}_{0,\tau}$.
The approximation of $\tilde{A}_t^{M^{(2n+2)}}$ is achieved by minimizing the following loss function:
\begin{equation} \label{eq:Loss of backward Markov prjection}
    \mathcal{L}(\phi)=\int_0^\tau \mathbb{E}_{\Lambda_{0, t}}\left[(\tilde{A}_t^{\mathbb{Q}_{\cdot \vert 0}} - \tilde{A}_t^{M^\phi})(X_t, X_t) + \sum_{y\ne X_t}\tilde{A}_t^{\mathbb{Q}_{\cdot \vert 0}}\log{\frac{\tilde{A}_t^{\mathbb{Q}_{\cdot \vert 0}}}{\tilde{A}_t^{M^\phi}}}(X_t, y)\right]dt,
\end{equation}
where $\tilde{A}_t^{\mathbb{Q}_{\cdot \vert 0}}$ denotes the time-reversal generator of pinned down process of $\mathbb{Q}(\cdot\vert X_0)$, and $\phi$ represents the parameters of the neural network approximating the time-reversed generator $\tilde{A}_t^{M^\phi}$.

In this manner, the iterative Markov projection following the reciprocal projection is performed alternately in a forward and backward (time-reversal) fashion.
Finally, this process yields a sequence of measures $(\Lambda^{(n)})_{n\in\mathbb{N}}$ and $(M^{(n)})_{n\in\mathbb{N}^+}$, which converges to $\mathbb{P}^\text{SB}$ in theory.

\subsection{Process on the Graph} \label{subsection:process on molecular graph}
We present a method for applying the previously described solution to a graph transformation.
A graph is represented as $\mathbf{G}=(\mathbf{V},\mathbf{E})$, where $\mathbf{V}=(v^{(i)})_{i}$ and $\mathbf{E}=(e^{(ij)})_{ij}$ denote node and edge features, respectively.
In a molecular graph, for example, the node and edge features correspond to atomic types and edge features, respectively.
Here, $\mathbf{V}$ and $\mathbf{E}$ are modeled as products of categorical random variables.

As the reference process, we define a jump process in which the nodes and edges of the graph change discretely, assuming that all nodes and edges are independent. 
Therefore, the transition probability $P$ and the rate $A$ of the reference process is described as follows:
\begin{align} \label{eq:CTMC graph}
    &P_{s:t}^{\mathbf{G}}(\mathbf{G}_1, \mathbf{G}_2)=\prod_{i} P_{s:t}^{V}(v_1^{(i)}, v_2^{(i)})\prod_{i,j}P_{s:t}^E (e_1^{(ij)}, e_2^{(ij)}), \nonumber \\
    &\partial_t P_{s:t}^{(\cdot)}(x, y) = \sum_{z\in\mathcal{X^{(\cdot)}}} P_{s:t}^{(\cdot)}(x, z)A_{t}^{(\cdot)}(z, y),\\
    &A^{(\cdot)}_s(x, y)=\partial_t P_{s:t}^{(\cdot)}(x, y)\big\vert_{t=s}, \nonumber
\end{align}
where $\cdot$ denotes $V$ or $E$, $\mathbf{G}_1$ denotes $(\mathbf{V}_1,\mathbf{E}_1)=\left((v_1^{(i)}), (e_1^{(ij)})\right)$, $\mathbf{G}_2$ denotes $(\mathbf{V}_2,\mathbf{E}_2)=\left((v_2^{(i)}), (e_2^{(ij)})\right)$, and $\mathcal{X}^V$ and $\mathcal{X}^E$ denote the state space of the nodes and edges, respectively.
More specifically, we use a monotonically decreasing function for signal to noise ratio, $\bar{\alpha}: [0, \tau] \to (0, 1]$, in which the transition rate is defined as:
\begin{equation} \label{eq:practical transition rate design}
    A_t^{(\cdot)}(x, y)=\partial_{t}(\ln{\bar{\alpha}}(t))\left(\delta_{xy}-\mathbf{m}^{(\cdot)}(y)\right),
\end{equation}
where $\delta_{xy}$ denotes the Kronecker delta, and $\mathbf{m}^{(V)}$ and $\mathbf{m}^{(E)}$ denote the prior distribution of nodes and edges as proposed in the previous discrete diffusion work \citep{vignac2022digress}.
According to the Kolmogorov equation, we get the transition probability as,
\begin{equation} \label{eq:practical transition probability design}
    P_{s:t}^{(\cdot)}(x,y)= \frac{\bar{\alpha}(t)}{\bar{\alpha}(s)}\delta_{xy} + \left( 1 - \frac{\bar{\alpha}(t)}{\bar{\alpha}(s)}\right)\mathbf{m}^{(\cdot)}(y).
\end{equation}

Note that the choice of $\mathbf{m}(\cdot)$ as uniform is associated to the diffusion on the state space $\mathcal{X}$, where the $\mathcal{X}$ is considered fully-connected graph. 
Moreover, the stationary distribution of the associated generator always becomes $\mathbf{m}(\cdot)$.
Although non-uniform choice of $\mathbf{m}(\cdot)$ breaks the diffusion formulation on $\mathcal{X}$, it does not harm SB formulation.


\subsection{Graph Permutation Matching}
\label{subsection:graph permutation matching}

The transition probability of the reference process depends on graph permutations (see \cref{eq:CTMC graph}), so graph permutation matching must be considered beforehand. 
Although this issue does not affect the sampling phase, it becomes problematic when computing the likelihood of the reference process for two given graphs $\mathcal{G}$ and $\mathcal{G}^\prime$, or when constructing a reciprocal process, which is a mixture of Markov bridges between the two graphs (see \cref{appendix.b.Graph permutation matching}).

One way to handle this is selecting a graph permutation that maximizes the likelihood under the reference process. 
Finding the optimal permutation can be formulated as a quadratic assignment problem (QAP), where the objective is to minimize the negative log-likelihood (NLL), consisting of the sum of the NLLs for both the nodes and edges.
While exact solutions are possible through mixed integer programming, the problem is NP-hard, so alternative methods are preferred.
Specifically, we employ a max-pooling algorithm by \citet{cho2014finding}, which is an approximation method categorized by continuous relaxation.
After obtaining an approximate solution, we use the Hungarian algorithm to discretize the assignment vector to the final solution.
We observed that the graph matching is highly accurate in molecular graph matching (see \cref{appendix.b.performance of graph matching algorithm}).
The details of the algorithm are described in \cref{appendix.b.solution method}.
We utilized the graph matching algorithm for every reciprocal bridge construction and likelihood computation.

Recall that the SB problem could be interpreted to the EOT problem, where the cost function corresponds to the NLL.
Thus, defining the reference process can be interpreted as defining a distance (cost) on the set of graphs.
Interestingly, we found that the likelihood of optimal permutation is interpreted as the graph edit distance (see \cref{appendix.b.relation to GED}).
This leads to the conclusion that the SB problem, with the $\mathbb{Q}$ as \cref{eq:practical transition probability design}, is analogous to an OT problem over the metric space of graphs equipped with graph edit distance as metric (GED), where the GED computation is well known to be NP-hard problem.

==> 06_results_and_discussion.tex <==
\section{Results and Discussions}
Here, we demonstrate the effectiveness of the Discrete Diffusion Schr\"odinger Bridge Matching (DDSBM) framework on graph transformation tasks.
Specifically, we apply DDSBM to a chemical domain, where the graph transformation task is nontrivial due to additional constraints imposed by molecular graphs and their associated properties.
We conducted experiments on two different molecule datasets: ZINC250K \citep{kusner2017ZINC250K} and Polymer \citep{StJohn2019}.
Throughout this section, we first elaborate on the common experimental setups and metrics for evaluation.
The second and third sections provide a detailed analysis of ZINC250K and Polymer experiments.
% ICLR
\ifthenelse{\boolean{isICLR}}{
    % isICLR이 true일 경우 이 섹션이 포함됨
    Finally, we empirically show utilizing an initial coupling based on the Tanimoto similarity \citep{willett1998chemical}, the widely-used metric for assessing chemical similarity, is effective for training DDSBM.
}{
    % isICLR이 false일 경우 이 부분은 비워둠
}

\subsection{Experimental setup and metrics}
\label{subsection: Experimental setup and metrics}

\textbf{Experimental Setup.} To train the models on graph transformation problems, an initial coupling between two distributions is necessary.
We randomly coupled the data of initial and terminal distributions to obtain paired data.
The molecular pairs are divided into training and test datasets in a ratio of 8:2.
The effect of different initial couplings is discussed in \cref{subsection:The effect of initial coupling}.
Detailed explanations about model architectures and hyperparameters can be found in \cref{appendix.c.Implementation details}.

\textbf{Metrics.}
By definition of SB (see \cref{eq:1 DSB definition}), both joint distribution and marginal distributions at each side must be examined to assess the degree to which the SB has been successfully achieved.
Specifically, we evaluate these distributions from two perspectives: graph structure and molecular properties.
While graph structure provides valuable insights, it alone may not be sufficient for molecular optimization tasks.
Therefore, the assessment of molecular properties is essential for a more comprehensive validation of the models, as these properties might exhibit weak correlations with the graph structures.

In the context of graph structure, we calculate Fréchet ChemNet Distance (FCD) score \citep{preuer2018frechet} between the target molecule distribution and the generated molecules from each model, which focuses on the marginal distribution of the molecules.
As the metric for evaluating the quality of the joint distribution, we report the negative log-likelihood (NLL), which measures the cost of transforming one graph into another based on the reference process, aligning with the graph edit distance (GED) (see \cref{appendix.b.relation to GED}).

For molecular properties, we measure the Wasserstein-1 distance ($W_1$) between the property distributions of the target and generated molecules representing the properties to be modified, which corresponds to the marginal distribution. 
In terms of the joint distribution, we calculate the mean absolute difference (MAD) of other key properties between the initial and generated molecules that should be retained, where drug-likeness (QED) \citep{bickerton2012quantifying} and synthetic accessibility score (SAscore) \citep{ertl2009estimation} are typical examples in optimizing drug candidates.

\subsection{Small molecule transformation}
\label{subsection:Small molecule transformation}
% 1. ZINC experiment
First, we validate our proposed methods on the SB problem between two molecule distributions constructed from the standard ZINC250K dataset.
We constructed two sets of molecules whose $\log{P}$ values are largely different.
Molecules from the ZINC250K dataset were randomly selected and divided into two sets whose $\log{P}$ values follow the Gaussian distributions centered at 2 and 4 with variance of 0.5, respectively (For more details, see \cref{appendix.ZINC250K-preprocessing}).
% More details can be found in \cref{appendix.ZINC250K-preprocessing}.
We compared our methods with three baseline models that perform graph-to-graph translation.
AtomG2G and HierG2G are latent-based models that encode an input graph into a latent vector and decode it into another graph \citep{jin2020HierG2G}.
Diffusion Bridge Model (DBM) is a bridge model trained with the same reference process as DDSBM, which is equivalent to the first Markov projection in DDSBM.
We refer readers to \cref{appendix.c.2.NeuralNetwork} for more details about the baselines and implementation of our models.
We note that, for these three baseline models, the initial coupling is utilized during the whole training procedure without change, while DDSBM dynamically alters the training data pair by Iterative Markovian Fitting (IMF).

\input{Tables/main_table_1_1}

\Cref{tab:main_table_1_1} shows overall results of our method compared to the three baseline models.
From \cref{tab:main_table_1_1}, we find that DDSBM constantly outperforms the other models in terms of both FCD and NLL.
% regardless of the initial coupling.
The lower FCD suggests that DDSBM-generated molecules are more similar to those in the target dataset, while the minimal NLL indicates that DDSBM applies minimal structural change on initial graphs.
This result demonstrates that DDSBM achieves more \textit{optimal} graph transformation between fixed initial and terminal distributions.
When it comes to the model type, bridge models achieved lower FCD and NLL compared to the latent-based models.
The bridge models, DBM and DDSBM, dynamically transform a graph based on the reference dynamics, favoring the retention of the given structure, whereas whole-graph reconstruction using a latent vector does not.
This leads to lower NLL values for the bridge models, which is ensured by the \cref{def:Markov projection}.
Additionally, the lower FCD values of the bridge models highlight that constructing a dynamic bridge within the graph domain enhances the performance of distribution learning for the target distribution.
Furthermore, we attribute the best performance of DDSBM to the gradual updating of training pairs, which become more similar than the random initial pairs, simplifying the graph transportation process.

Next, we analyze molecular properties of the source and generated molecules.
DDSBM resulted in the lowest MAD in QED and SAscore, meaning deviation of molecular properties other than $\log{P}$ is the smallest for DDSBM.
It is noteworthy that DDSBM achieves minimal changes in various molecular properties despite being trained solely to optimize graph transformations with minimal structural alterations, without explicit knowledge on molecular properties.
Meanwhile, the latent-based models exhibited larger MAD values in QED and SAscore, indicating they are vulnerable to losing other properties of the initial molecules.
This can be inferred from the result of HierG2G; although HierG2G achieves the lowest $W_1$ value in $\log{P}$ so that it modulates $\log{P}$ the best to the desired degree,  its much larger NLL value suggests that it might generate a graph with less consideration of the initial graph constraint, as illustrated in \cref{figure:figure1}.
For a better understanding of overall results, we provide the corresponding distributions of properties of the models in \cref{figure:figure_distributions}.

% Connection to 5.4
Despite the promising results, we observe that all models except DDSBM have a high reliance on a pre-defined initial coupling.
Thus, we conducted additional experiments using pseudo-optimal initial coupling based on Tanimoto similarity, which is detailed in \cref{subsection:The effect of initial coupling}.
Interestingly, we found that introducing the pseudo-optimal initial coupling not only accelerated the training of DDSBM in practice but also allowed it to achieve performance on par with the previous results.

% ICLR
\ifthenelse{\boolean{isICLR}}{
    % isICLR이 true일 경우 이 섹션이 포함됨
}{
    % isICLR이 false일 경우 이 부분은 비워둠
}

% 2. Polymer dataset
% polymer: S1 <- prediction model (molclr finetuning) / NLL
% no baseline % case-study
\subsection{Polymer graph transformation}
\label{subsection:Polymer graph transformation}
The Polymer dataset \citep{StJohn2019} consists of 91,000 monomer molecules with their optical excitation energies (GAPs) obtained by time-dependent density functional theory calculations.
We reconstructed the Polymer dataset for a transport problem between two sets of molecules with distinct GAPs, corresponding to green and blue optical colors, respectively.
The reconstructed dataset contains 7,603 molecular pairs.
This task is considered as a more challenging application because the relationship between the graph structure and the target GAP property is highly non-linear, making it hard to predict the effect of specific structural changes on the GAP.
In this context, we apply our DDSBM model to find the optimal transformation between the two sets of molecules.

The performance of DDSBM is compared to DBM, which serves as a baseline.
The GAPs of the molecules generated by the models were obtained using the pre-trained MolCLR model \citep{wang2022molecular}, which has a mean absolute error (MAE) of 0.027 eV for the GAP prediction.
\Cref{tab:main_table_2_1} shows the overall results of our method on the Polymer dataset.
Apparently, DDSBM outperforms DBM on all evaluated metrics, which is consistent with the results from the experiments on ZINC250K.
In terms of validity, DBM shows significantly lower scores, which contrasts with the results observed on the ZINC250K dataset.
This can be attributed to the characteristics of the molecules in the Polymer dataset, which have relatively large sizes and multiple ring structures.
In this context, minimal transformations are advantageous for achieving high validity, and DBM may have struggled to learn these changes from the randomly paired data.
Examples of the generated molecular graphs are visualized in \cref{figure:figure_polymer}.

\input{Tables/main_table_2_1}

% Comment this for ICLR
\ifthenelse{\boolean{isICLR}}{
    \input{200_result_5_4}
}{
}

==> 200_result_5_4.tex <==
\subsection{The effect of initial coupling}
\label{subsection:The effect of initial coupling}
We further analyze the molecular optimization task in \cref{subsection:Small molecule transformation} with different initial couplings.
In that section, we used randomly coupled molecules as the initial coupling for all the models.
However, except for DDSBM, all of them assume that suitable molecule pairs have already been identified to be provided.
To meet this, we adopted Tanimoto similarity \citep{willett1998chemical} as a pseudo-metric to find similar molecule pairs between the two molecule distributions, denoted as Tanimoto similarity-based coupling.
We note that the similarity-based coupling is another optimal transport problem of \textit{maximizing} the sum of pair-wise molecular similarities, where we employed the Hungarian method to obtain a sub-optimal solution.

Using the Tanimoto similarity-based coupling, we retrained all models discussed in \cref{subsection:Small molecule transformation} and compared their performance.
Here, we denote a newly trained DDSBM model as DDSBM-T to deviate it from the model trained on the randomly coupled data.
From \cref{tab:main_table_3}, we observe that all models achieved lower NLL values compared to when they were trained with random coupling.
The HierG2G model exhibits much lower FCD and NLL values compared to those of random coupling, indicating that previous graph transformation methods can be improved if more optimal pairs are provided as training data.

The distinct feature of DDSBM-T is that all baseline models learn graph transformations between the molecule pairs with high Tanimoto similarity, while DDSBM-T learns graph transformations with minimal cost defined by its reference process $\mathbb{Q}$.
\input{Figures/main_figure_2}
It cannot be guaranteed that the distance defined by our reference process is better than the Tanimoto similarity from the perspective of molecular optimization.
Essentially, the success of molecular optimization should be measured by how well the target property is adjusted while preserving other key properties.
Apparently, \cref{tab:main_table_3} shows that DDSBM-T outperforms the other baselines in terms of molecular property metrics.
This suggests that the graph transformation from DDSBM retains other molecular properties, attaining the goal of the molecule optimization task.


Finally, we analyze the effect of initial coupling on the training process, especially focusing on the approach to convergence.
We illustrate the training losses of DDSBM models from two different initial couplings, random and Tanimoto similarity-based, in \cref{fig:figure2}, respectively.
DDSBM-T shows consistently lower loss values up to the sixth IMF iteration and reaches convergence at the third IMF iteration.

% 1. 물성 성능
\input{Tables/rev_main_table_3}

==> Tables/main_table_1.tex <==
\begin{table}[h!]
\caption{
% Caption PlaceHolder
% EXP SETTING: Random pair Uniform $\bar{\alpha}_T$ 0.95
\textbf{Distribution shift performance on ZINC.}
The reference FCD is computed with test source molecules and training target molecules.
$\uparrow$ and $\downarrow$ denote higher and lower values are better, respectively.
}
\centering
% VAL, FCD, NLL, Original NLL
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule

\multirow{2.5}{*}{Model}
& \multirow{2.5}{*}{Type}
& \multicolumn{3}{c}{Random initial coupling}
& \multicolumn{3}{c}{Tanimoto initial coupling}
\\

\cmidrule(lr){3-5} \cmidrule(lr){6-8}

% PLACE HOLDER
& %
& Validity$(\uparrow)$
& FCD$(\downarrow)$
& NLL$(\downarrow)$
& Validity$(\uparrow)$
& FCD$(\downarrow)$
& NLL$(\downarrow)$
\\

\midrule

Reference
& -
& -
& 4.807
& 361.244
& -
& 4.812
& 242.232
\\

\midrule

AtomG2G
& Latent
& \textbf{100.0}
& 5.474
& 347.675
& \textbf{100.0}
& 5.665
& 347.758
\\

HierG2G
& Latent
& \textbf{100.0}
& 4.384
& 344.869
& \textbf{100.0}
& 1.150
& 263.125
\\

\midrule

DBM
& Bridge
& 88.9
& 1.542
& 258.517
& 87.2
& \textbf{0.755}
& 225.583
\\

DDSBM
& Schrödinger Bridge
& 95.9
& \textbf{0.880}
& \textbf{160.816}
& 94.5
& 0.932
& \textbf{156.542}
\\

\bottomrule
\end{tabular}
}
\label{tab:main_table_1}
\end{table}


==> Tables/main_table_1_1.tex <==
\begin{table}[t!]
\caption{
% EXP SETTING: Random pair Uniform $\bar{\alpha}_T$ 0.95
\textbf{Distribution shift performance on ZINC.}
Reference refers to metrics from the initial coupling, used as a standard to evaluate each model’s graph translation.
For both AtomG2G and HierG2G, we've excluded the generated molecules that are too large with more atoms than the maximum number of atoms in our dataset for computing metrics other than validity.
$\uparrow$ and $\downarrow$ denote higher and lower values are better, respectively.
The best performance is highlighted in bold.
}
\centering
% VAL, FCD, NLL, Original NLL
\resizebox{1.0\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{lc|ccc|ccc}
\toprule

Model
& Type
& Validity$(\uparrow)$
& FCD$(\downarrow)$
& NLL$(\downarrow)$
& LogP $W_1(\downarrow)$
& QED MAD$(\downarrow)$
& SAscore MAD$(\downarrow)$
\\

\midrule

Reference\tnote{1}
& -
& -
& 4.807 / 0.279
& 360.862
& 2.007
& 0.153
& 0.595
\\

\midrule

AtomG2G
& Latent
& \textbf{100.0}
& 5.480
& 347.280
& 0.222
& 0.135
& 0.742
\\

HierG2G
& Latent
& \textbf{100.0}
& 4.413
& 344.208
& \textbf{0.053}
& 0.135
& 0.657
\\

\midrule

DBM
& Bridge
% IMF Iteration 5
% & 88.9
% & 1.542
% & 258.517
% & 0.126
% & 0.123
% & 0.583
% IMF Iteration 6
& 89.5
& 1.038
& 285.576
& 0.161
& 0.145
& 0.611
\\

DDSBM
& Schrödinger Bridge
% IMF Iteration 6
& 95.3
& \textbf{0.896}
& \textbf{162.228}
& 0.134
& \textbf{0.118}
& \textbf{0.398}
\\

\bottomrule
\end{tabular}

\begin{tablenotes}
\footnotesize
\item[1] NLL, $W_1$, and MADs were calculated using random pairs from the test set. Two FCD values are provided: the first compares the initial molecules in the test set with the terminal molecules in the training set, and the second compares the terminal molecules in both sets.
\end{tablenotes}
\end{threeparttable}
}
\label{tab:main_table_1_1}
\end{table}


==> Tables/main_table_2.tex <==
\begin{table}[h!]
\caption{
\textbf{Molecular optimization performance on ZINC.}
$\downarrow$ denotes lower values are better.
}
\centering
% VAL, FCD, NLL, Original NLL
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule

\multirow{2.5}{*}{Model}
& \multirow{2.5}{*}{Type}
& \multicolumn{3}{c}{Random initial coupling}
& \multicolumn{3}{c}{Tanimoto initial coupling}
\\

\cmidrule(lr){3-5} \cmidrule(lr){6-8}

% PLACE HOLDER
& %
& LogP $W_1(\downarrow)$
& QED MAD$(\downarrow)$
& SAscore MAD$(\downarrow)$
& LogP $W_1(\downarrow)$
& QED MAD$(\downarrow)$
& SAscore MAD$(\downarrow)$
\\

\midrule

Reference
& -
& 2.007
& 0.153
& 0.595
& 2.011
& 0.126
& 0.367
\\

\midrule

AtomG2G
& Latent
& 0.222
& 0.135
& 0.742 
& 0.220
& 0.136
& 0.739
\\

HierG2G
& Latent
& \textbf{0.064}
& 0.136
& 0.662
& 0.200
& 0.129
& 0.448
\\

\midrule

DBM
& Bridge
& 0.126
& 0.123
& 0.583
& 0.157
& 0.134
& 0.565
\\

DDSBM
& Schr\"odinger Bridge
& 0.118
& \textbf{0.115}
& \textbf{0.398}
& \textbf{0.140}
& \textbf{0.117}
& \textbf{0.382}
\\

\bottomrule
\end{tabular}
}
\label{tab:main_table_2}
\end{table}


==> Tables/main_table_3.tex <==
\begin{table}[h!]
\caption{
% EXP SETTING: Random pair Uniform $\bar{\alpha}_T$ 0.95
\textbf{Distribution shift performance on ZINC with initial coupling based on the Tanimoto similarity.} As in \cref{tab:main_table_1_1}, reference refers to metrics from the initial coupling, used as a standard to evaluate each model’s graph translation. The experimental setting is the same as described \cref{subsection:Small molecule transformation}, except for the initial coupling. 
}
\centering
% VAL, FCD, NLL, Original NLL
\resizebox{1.0\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{lc|ccc|ccc}
\toprule

Model
& Type
& Validity$(\uparrow)$
& FCD$(\downarrow)$
& NLL$(\downarrow)$
& LogP $W_1(\downarrow)$
& QED MAD$(\downarrow)$
& SAscore MAD$(\downarrow)$
\\

\midrule

Reference\tnote{1}
& -
& -
& 4.811 / 0.315
& 245.765
& 2.011
& 0.126
& 0.367
\\

\midrule

AtomG2G
& Latent
& \textbf{100.0}
& 5.676
& 346.499
& 0.220
& 0.136
& 0.738
\\

HierG2G
& Latent
& \textbf{100.0}
& 1.171
& 264.072
& 0.189
& 0.127
& 0.446
\\

\midrule

DBM
& Bridge
% IMF iteration 6
& 90.2
& \textbf{0.749}
& 220.594
& 0.141
& 0.127
& 0.508
\\

DDSBM-T
& Schrödinger Bridge
& 95.6
& 0.911
& \textbf{152.856}
& \textbf{0.103}
& \textbf{0.110}
& \textbf{0.393}
\\
% compile 에러 고쳐주세요
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] NLL, $W_1$, and MADs were calculated using random pairs from the test set. Two FCD values are provided: the first compares the initial molecules in the test set with the terminal molecules in the training set, and the second compares the terminal molecules in both sets.
\end{tablenotes}
\end{threeparttable}
}
\label{tab:main_table_3}
\end{table}

